Manifold-Kernels Comparison in MKPLS for Visual Speech Recognition

Speech recognition is a challenging problem. Due to the acoustic limitations, using visual information is essential for improving the recognition accuracy in real-life unconstraint situations. One common approach is to model the visual recognition as nonlinear optimization problem. Measuring the distances between visual units is essential for solving this problem. Embedding the visual units on a manifold and using manifold kernels is one way to measure these distances. This work is intended to evaluate the performance of several manifold kernels for solving the problem of visual speech recognition. We show the theory behind each kernel. We apply manifold kernel partial least squares framework to OuluVs and AvLetters databases, and show empirical comparison between all kernels. This framework provides convenient way to explore different kernels.

==> databases_old.tex <==
\subsection{Databases}
\label{sec:databases}
%There are many databases available for AVSR, such as AVLetters \cite{Matthews2002-avletters}, AVLetters 2 \cite{Cox2008-AVLETTERS2}, AVICAR \cite{Lee2004-AVICAR}, AV-TIMIT \cite{Hazen2004-AVTIMIT}, GUAVE \cite{Patterson:2002} and OuluVS \cite{Zhao2009}. All AVSR databases can be used for VSR research by simply ignoring the audio information. Our choice  is based on several factors. First, we are looking for recent work using solely visual data to compare with. Second, we need to test on different length spoken units. Third, reasonable image resolution. 

We use the same databases used in \cite{Bakry2013}: AVLetters \cite{Matthews2002-avletters}  and OuluVs \cite{Zhao2009}. % for speech recognition and speaker identification. 
In all experiments, the recognition rate is measured as the ratio between the correctly recognized clips and the total number of clips.
\vspace{-12px}

\paragraph*{AVLetters database} \cite{Matthews2002-avletters} has ten subjects. Each speaker repeats every English letter ($A\cdots Z$) exactly three times, with a total of $780$ video sequences. The speaker was requested to start and end utterance of every letter in a neutral state (mouth closed). No head motion/rotation is allowed from speakers. Every frame is a $60\times 80$ pixel %s of moderate resolution
image of the mouth area. %This database is very challenging for VSR. The best achieved accuracy for recognizing the spoken letter has been on this database is about $62\%$ \cite{Zhao2009}. 
We use the following setting:
For $\mathbf{LBP}$ features, we tried many configuration. The results is reported in terms of two of them: single cell eight-resolutions ($\mathbf{LBP}_{1:8\times 8}$) and $3\times 4$ cell-grid  with four-resolutions ($_{3\times 4}\mathbf{LBP}_{1:4\times 8}^{u_2}$). For more details about \textbf{LBP}, reader is referred to \cite{Ojala2002}.
\vspace{-12px}
\paragraph*{OuluVS database} \cite{Zhao2009} it consists of ten different everyday phrases. Each phrase is uttered by $20$ subjects up to five times. The frame rate was set to $25$ fps. The dataset  contains sequence of images for mouth area with average resolution of $120 \times 60$ pixels. This database is less constrained than AVLetters, so that limited rotation and shift was allowed in the recording time, %Figure~\ref{fig:ouluvs_examples}(\textbf{a}). %slightly shiftedIn this area, you can find some mouthes slightly rotated and shifted. 
%Not all sequences are perfectly segmented, so that, some sequences have few frames with partial-mouth (Figure~\ref{fig:ouluvs_examples}(\textbf{b})) or non-mouth frames (Figure~\ref{fig:ouluvs_examples}(\textbf{c})). 
%Some of the outlier sequences (that contain very few mouth/partial-mouth frames) are excluded from the experiment. Consequently, we exclude four speakers with very few sequences remaining (\textit{P004}, \textit{P005}, \textit{P010} and \textit{P016}).
%
%\begin{figure}
%\begin{tabular}{c c c}
%\includegraphics[width=0.4\columnwidth]{figs/ouluvs_complete}&
%\includegraphics[width=0.2\columnwidth]{figs/ouluvs_partial}&
%\includegraphics[width=0.2\columnwidth]{figs/ouluvs_nonmouth}\\
%(\textbf{a}) & (\textbf{b})& (\textbf{c})\\
%\end{tabular}
%\caption{OuluVs: (\textbf{a}) Regular frames, (\textbf{b}) Partial mouth area frames, (\textbf{b}) Non-mouth area frames.}
%\label{fig:ouluvs_examples}
%\vspace{-10px}
%\end{figure}
The feature configurations used on this database is  %($\mathbf{LBP}_{1:8\times 8}$) and 
($_{1\times 2}\mathbf{LBP}_{1:8\times 8}^{u_2}$).


==> experiments_copy.tex <==

\subsection{Experimental Results}
In this section, we present the empirical results of MKPLS when plugined with each one of the kernels described in Section~\ref{sec:kernels}. To give real comparison between the proposed kernels, we need to explore different parameters of MKPLS pipeline:
The number ($n$) of Gaussain-RBF basis $\psi$ that we use to learn the individual manifold parameterization, we show results for $n={8,16}$.
%Parameter affects the generation of the manifold parameterization which is the number of temporal centers $n$. 
The dimensionlaity of the manifold latent space, we use $m = {10,30,50,80,100,130,200}$, which cover wide range of the possible values.

Especially for Grassmann-based kernels~\ref{sec:kernels}, we show the affect of using the parameterization of the LBP of the images itself vs LBP of the images concatenated with parameterization of the discrete difference between those images.
%This section is organized by experiment protocoals and within each experiment we compare using different kernels.

\subsubsection{Visual speech recognition}
Two test protocols has been adopted for visual speech recognition: Speaker Independent (SI) and Speaker Semi-Dependent (SSD) as defined in ~\cite{Bakry2013}.
%, we had one more protocol "speaker dependent", but we skipped it here, because we need to measure the ability of the framework to balance between the speaker and speech variations. For each configuration, we are going to show the result of the set of kernels discribed in Section~\ref{sec:kernels}.
\paragraph*{Speaker Semi-Dependent VSR (SSD):} Here we test on one repeat of the available videos and train based on the remaining repeats for the same subjects. In this configuration all subjects and phrases are presented in the training set. %The challenge here is to classify the phrase correctly regardless the user identity.
Table~\ref{fig:ouluvs-SSD} show the SSD speech recognition accuracy for OuluVs for the two feature configurations.
\paragraph*{Speaker Independent VSR (SI):} the challenge here is %to recognize the uttered phrase, independent of the speaker. By this configuration. 
to show the scalability of the model, mean how far the model can recognize the spoken phrase based on the dynamics even if the speaker is not seen before in the training set. In this experiment, we use one-speaker-out. Table~\ref{fig:ouluvs-SI} show the SI speech recognition accuracy for OuluVs for the two configurations.
\subsubsection{Speaker Identification (SpId):}
The goal in this experiment is to find the speaker within the register set of users. The challenge is to find the speaker from the limited available information in the mouth area. 
%Moreover, we want to prove that although the manifold parameterization encodes mainly the geometric deformation from the unified manifold to the original data manifold, parameterization also hold speaker-related information. 
We take one repetition out for testing, and train over all other repetitions.
Table~\ref{fig:ouluvs-speaker} shows the speaker identification accuracy when applied to OuluVs for the two test configurations.



==> framework.tex <==
\subsection{Problem Definition}
\label{sec:problemDef}
Given set of visual units, we need to recognize new test unit, and infer the identity of the speaker. The visual unit could be viseme, word or a complete sentence. For each training visual unit is assigned to specific speech class and specific speaker. %  to group them semantically by human perceiption of them. 
Both the training and testing visual units are represented by sequence of images (frames) extracted from the speech video. Each frame exposes only the mouth area of the speaker. % The frames are restricted to mouth area for the biometric and privacy reasons.
%We have a set of images sequences representing different visual units. 
\subsection{Framework description}
\label{sec:framework}
Manifold Kernel Partial Least Squares (MKPLS) framework is proposed in \cite{Bakry2013}. For convenience, we briefly describe the mathematical model and the framework pipelines here.%in this section.
%
%\subsection{Mathematical model}
%\textbf{Mathematically,}
Let us denote the $k$-th sequence by  $S_k= \{ \vect{x}^k_i \in \mathbb{R}^D, i=1\cdots n_k \}$, 
where the image $\vect{x}^k_i\in \mathbb{R}^D$. Let $y_k$ represents the class labels for the $k$-th sequence. For the particular case of speech recognition and speaker identification, $y_k\in \{c_1, \cdots, c_K\} \times \{p_1, \cdots p_L \}$.  Here $c_i$ is the speech label, and $p_j$ is the performer identity. 
%
Let $\mathcal{M}_k\subset \mathbb{R}^D$ is a low-dimensional manifold connects the images of sequence $S_k$.  The basic assumption is that all these manifolds ($\mathcal{M}_k \forall k$) are topologically equivalent, however each of them has different geometry in $\mathbb{R}^D$. This assumption is stated clearly in \cite{Bakry2013}. %In other words, all these manifolds are deformed instances of each others. This assumption is fairly met in the domain of activity recognition. For example, periodic locomotive activities intuitively lie on one-dimensional closed manifolds, and hence topologically equivalent.  For instance, sequence of features representing a Viseme, starting from a neutral pose and reaching a peak pose, lies on a one-dimensional manifold (curve) in the feature space. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We use this framework for evaluating the performance of all manifold kernels that we discuss in this paper. 

 %Fourth, this framework uses kernel based dimensionality reduction technique which gives the ability to investigate different manifold kernels. 
%
%
In principal, \textbf{MKPLS pipeline} has three phases: individual manifold parameterization, latent space embedding and finally inference/classification. 
%
Consider the manifold $\mathcal{M}_k$ connects the $n_k$ frames of specific Visual Unit (VU).  Assuming, that we have a unified manifold $\mathcal{U}$.
%
%MKPLS represents each visual unit in manifold formate, and 
The result of \textbf{individual manifold parameterization} is a single representation for VU which holds the topological deformation of $\mathcal{M}_k$ with respect to $\mathcal{U}$. Any further processing is done based on these parameterizations. % This step minimizes the effect of the temporal variations between visual units. 
%
%
The manifold $\mathcal{M}_k$ is represented by a parameterization $\mathbf{C}_k$ with respect to a set of basis $\{\psi_1,\psi_2,\cdots,\psi_n\}$. These basis are a nonlinear function of points on $\mathcal{U}$. We use Gaussian Radial Basis Function (Gaussian-RBF):
$\psi_{i}(\vect{z})=exp(\sigma\left\|\vect{z}-\vect{w}_i\right\|)$
%\begin{equation}
% \label{eq:gaussian-rbf-psi}
% \psi_{i}(\vect{z})=exp(\sigma\left\|\vect{z}-\vect{w}_i\right\|)
% \end{equation}
where $\vect{w}_i; i =1\cdots n$ are fixed points on $\mathcal{U}$.
%
%[K(\vect{z},\vect{w}_1), \cdots, K(\vect{z},\vect{w}_n)]$ . 
The goal is to find a regression function $\mathcal{\gamma}(t) = \mathbf{C}_k^\top \Psi(t)$ which minimize the objective function  %$\mathcal{\gamma}(t) $ is chosen to minimizes a regularized loss functional in the form 
\begin{equation}
\label{eq:gamma}
    \sum_i^{n^k} \left\|\vect{x}^k_{i} - \gamma^k(\mathbf{z}^k_i)\right\|^2 + \lambda \; \Omega[\gamma^k], 
\end{equation}
where $\left\|\cdot\right\| $ is the Euclidean norm,  $\Psi(t)=[\psi_1(\vect{z}_t),\psi_2(\vect{z}_t),\cdots,\psi_n(\vect{z}_t)]^\top$, $\Omega$ is a regularization function that enforces the smoothness in the learned function, and $\lambda$ is the regularizer. %that balances between fitting the training data and smoothing the learned function. When $\lambda\to 0$, the regression function over-fits the training data. 
Representer theory helps to find closed form for $\mathbf{C}$ as
\begin{equation}
\label{eqn:coeff_matrix}
\mathbf{C}_k^\top  = (\mathbf{A}_k^\top\mathbf{A}_k+\lambda \mathbf{G})^{-1}\mathbf{A}_k^\top\mathbf{X}_k^\top, 
\end{equation}
where $\mathbf{A}_k$ is an $n_k \times n$ matrix with $\mathbf{A}_{(ij)}= exp(\sigma\left\|\vect{z}_i-\vect{w}_j\right\|)$ %, i=1, \cdots,n_k,  j=1 \cdots n$ 
and $\mathbf{G}$ is an $ n \times n$ matrix with $\mathbf{G}_{(ij)}=exp(\sigma\left\|\vect{w}_i-\vect{w}_j\right\|)$%;  i,j=1 \cdots n$
. $\mathbf{X}_k$ is the $n_k \times D$ data matrix for UV$_k$. The details of learning the manifold parameterization can be found in \cite{Bakry2013}. %Solution for $\mathbf{C}$ is guaranteed under certain conditions on the basis functions \cite{Poggio1990:GRBF}. In this paper, we use Gaussian Radial Basis Function (Gaussian-RBF) for the kernel $K(\cdot,\cdot)$.

The choice of $\lambda$ and $n$ is crucial for better performance. Figure~\ref{Fig:comapare-lambda-n} shows the trade-off between value of $\lambda$ and $n$. This choice depends upon the application. In this work, we need to capture the smooth dynamics in the visual units. Therefore, we choose $\lambda=50$. It is clear that $n=16$ expose more variations than with $n=8$. More information can be useful in some cases and can be more confusing in others. Threrefore, in Section~\ref{sec:experments}, we show both configurations.
\begin{figure}
%\centering{
\includegraphics[width=1.2\columnwidth]{figs/n_lambda_figure}
%}
\vspace{-15px}
\caption{The parameterization $C$ is $D\times n$ matrix. Each plot has $D$ lines, and each line is a plot for values progression of a row in $C$. At large values of $\lambda$ the parameterization is smooth enough to capture large dynamics in the visual unit.%For $n=16$ the parameterization holds more informatoin than for $n=8$
}
\label{Fig:comapare-lambda-n}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In \textbf{Latent space embedding}, kernel partial least squares (KPLS) \cite{Rosipal2002:KPLS}  is adopted for embedding the parameterizations $\{\mathbf{C}_k, k=1\cdots N\}$ into a low-dimensional latent space $\mathbb{R}^m$, as $\{\mathbf{t}_k\in \mathbb{R}^m, k=1\cdots N\}$. KPLS is supervised method, so it uses the set of labels $\{y_k, k=1\cdots N\}$ for the embedding. Supervised embedding guarantees to acheive the most concise and informative low-dimensional latent space embedding.
For any manifold $\mathcal{M}_\nu$, represented by its parameterization $\mathbf{C}_\nu$, the corresponding embedded point can be computed by
\begin{equation}
\label{eqn:embedding}
\mathbf{t_\nu = \mathbf{v}_\nu R}.
\end{equation}
Where the projection matrix $\mathbf{R}$ is learned from KPLS algorithm, and $\mathbf{v}_\nu=K(C_\nu,.)\in \mathbb{R}^N$. $K$ measures the similarity between $C_\nu$ and all training manifold parameterizations $\{\mathbf{C}_k, k=1\cdots N\}$.
The choice of kernel $K$ and its computation is discussed in detailed in Section\ref{sec:kernels}.
Because we solve two problems, speech recognition and speaker identification, we learn one $\mathbf{R}$ for each task. We learn $\mathbf{R}_c$ based on speech labels, and we learn $\mathbf{R}_p$ for speaker identification with subject labels. As a result, for each $\mathbf{v}_\nu$, we get two embedding in two latent spaces: $\mathbf{t}_\nu^c=\mathbf{v}_\nu \mathbf{R}_c$ in the speech latent space and $\mathbf{t}_\nu^p=\mathbf{v}_\nu \mathbf{R}_p$ in the speaker latent space.


%\begin{equation}
%\label{eqn:projection}
%\mathbf{T} = \mathbf{K}\mathbf{R}
%\end{equation} 
%Where $T$, of all embedded points, can be written as
%
%
%\subsection{Multifactor Embedding}
%As aforementioned, we have set of labeled manifold parameterizations $\{(\mathbf{C}_k,y_k);\ k=1\cdots N\}$. Consider the case where we have multiple labeling for the same manifold. Therefore, we need to deal with different classification tasks.
%% For instance, when we aim to recognize the uttered phrase, we need to label the manifolds by their phrase label. On the other hand, if we are doing speaker recognition, then manifolds have speaker labeling. In other word, manifolds have different labelings, according to different goals we need to achieve.
%In this paper, we have two simultaneous tasks: speech recognition and speaker identification.
%
%For phrase/speech recognition, the input manifolds have labeling $y^h_k, k=1\cdots N$. We can learn projection matrix $\mathbf{R}^h$ for embedded points $\mathbf{T}^h$ ({\textbf Algorithm~\ref{alg:kpls}}). 
%
%For any new manifold $\mathcal{M}_\nu$, $\mathbf{C}_\nu$ is compute (Eq~\ref{eqn:coeff_matrix}), then get the corresponding embedded point by Eq~\ref{eqn:embedding}, as $\mathbf{t}^h_\nu = \mathbf{v}_\nu \mathbf{R}^h$.
%
%For speaker identification, we have different labeling $y^p_k, k=1\cdots N$. Similarly, we learn the projection matrix $\mathbf{R}^p$ and the embedded points $\mathbf{T}^p$. For new manifold $\mathcal{M}_\nu$, we compute the parameterization $\mathbf{C}_\nu$, then get the corresponding embedded point by $\mathbf{t}^p_\nu = \mathbf{v}_\nu R^p$.
%

Finally in \textbf{manifold classification}, given a latent space embedding $\mathbf{t}_\nu$, MKPLS uses several techniques to classify it such as 
Regression for classification (RfC) \cite{Bakry2013}, Support vector machines (SVM) and K-nearest neighbor (KNN). In the latent space of speech, we want to infer the speech label ($c$) while in the speaker space, we need to infer the subject label ($p$). 

%Use regression results of KPLS
%\[
%%L_\nu = t_\nu T^\top\mathbf{L}
%\hat{y}_\nu = \mathbf{t}_\nu \mathbf{T}^\top\mathbf{y}
%\]
%where $t_\nu$ is computed from Eq~\ref{eqn:embedding} (details are in \cite{Bakry2013}). 
%Second choice is Support vector machines (SVM). A one-vs-all SVM classifier is learned using the set of training points $\{(\mathbf{t}_k,y_k)\in \mathbb{R}^m\times \mathbb{R};\ k=1\cdots N\}$.



%
%\section{Single frame classification}
%\section{Toward continuous speech recognition}
%In the section \ref{sec:classify}, we assumed that we have all frames of the new sequence $\mathcal{S}^\nu$ are avaialble. Toward continuous speech recognition, we have to consider the case of classifying the phrase/speaker from solely single or couple of frames. 
%
%For doing that, we need to have generative model. Recipe of generative model is 1) descriptor for single frame 2) some measurement for how sure we are that the image in hand belong to certain sequence 3) classifier for he choosen sequence to know the word and the speaker of this speech video.
%We can do that using sampling method. So we sample from both the 
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %


==> framework_old.tex <==
\section{Problem Definition}
\label{sec:problemDef}
We have a set of images sequences representing different visual units. The visual unit could be viseme, word or a complete sentence. Let us denote the $k$-th sequence by  $S_k= 
\{ \vect{x}^k_i \in \mathbb{R}^D, i=1\cdots n_k \}$, 
where the images are represented using suitable features of dimensionality $D$. Let $y_k$ represents the class labels for the $k$-th sequence. In this paper, for the particular case of speech recognition and speaker identification, $y_k\in \{c_1, \cdots, c_K\} \times \{p_1, \cdots p_L \}$.  Here $c_i$ is the activity class label (speech unit), while $p_j$ is the performer class label (speaker). Each sequence lies on a low-dimensional manifold, denoted by $\mathcal{M}_k$, embedded in the feature space $\mathbb{R}^D$. We will denote these manifolds by {\em instance manifolds}.  The basic assumption is that all these manifolds are topologically equivalent, however each of them has different geometry in $\mathbb{R}^D$. In other words, all these manifolds are deformed instances of each others. This assumption is fairly met in the domain of activity recognition. For example, periodic locomotive activities intuitively lie on one-dimensional closed manifolds, and hence topologically equivalent.  For instance, sequence of features representing a Viseme, starting from a neutral pose and reaching a peak pose, lies on a one-dimensional manifold (curve) in the feature space. 

%The goal is to achieve a low-dimensional latent space of instance manifolds. In that space each manifold is represented by a single point. Based on that space, instance classification can be achieved. We learn two classification functions $f_{speech}(S)$ and $f_{speaker}(S)$ based on two latent spaces for speech and speaker respectively.
%%The first step in our framework is to parameterize these manifolds to obtain a descriptor for each of them. Finding a good descriptor for objects/patterns is a crucial task in pattern recognition. Several holistic descriptors were devised and widely used for a given image, \eg GIST\~cite{GIST}, ~\cite{Ojala2002}. The manifold parameterization we using can be thought of as a holistic spatio-temporal descriptor of a whole sequence of frames representing an activity. 

%The first step in our framework is to parameterize these manifolds to obtain a descriptor for each of them. The manifold parameterization we use is based on~\cite{elgammal-chansu-cvpr04,Lee-elgammal-iccv05}. We learn a regularized mapping function from a unified (average) low-dimensional embedded representation of all manifolds to each input manifolds. These mapping functions encode the geometric deformations between the unified representation and the original data manifolds. 
%Therefore, the space of coefficients of these mapping functions provides a parameterization of the input manifold. 

%The obtained parameterization is high-dimensional, which makes it hard to learn classification functions that can generalize well. In~\cite{elgammal-chansu-cvpr04} subspace analysis was used to obtain a latent representation of the manifold parameterization space. However such approach does not benefit from available class labels.  Alternatively, we propose a supervised way to achieve a low-dimensional latent manifold parameterization space, which benefits from the class labels. Given the instance manifold parameterization, we propose two alternative manifold kernels based on the parameterization space. Given a manifold kernel, we use KPLS in the parameterization space to obtain a latent low-dimensional manifold parameterization space. We apply KPLS independently for the speech and speaker factors.


%It worth mentioning that the unified manifold representation is supposed to be topological equivalent to each instance manifold. This can not simply be obtained by traditional Dimensionality Reduction (DR) on the whole input data. This is because the goal of DR approaches is to find an embedding that preserves the local (or global) geometry of the data. In contrast, the unified manifold representation is a collapsing of all instance manifolds to one average manifold. There are various ways that can be used to achieve this. In~\cite{elgammal-chansu-cvpr04} individual manifolds are embedded and warped to compute an average embedding. Alternatively, if the topology of the manifold is known, a conceptual representation can be imposed; for example a unit circle can be used as topologically equivalent representation of all closed one-dimensional manifolds~\cite{Lee-elgammal-iccv05}. Another alternative is to use manifold alignment (\eg~\cite{Ham2005}) to learn a unified embedding.  In this paper, we work on top of such unified representation, independent of the approach used to achieve it. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Manifold-KPLS Framework}
\label{sec:framework}
Manifold Kernel Partial Least Squares (MKPLS) framework proposed in \cite{Bakry2013}. For convenience, we briefly describe it in this section. %We use this framework for evaluating the performance of all manifold kernels that we discuss in this paper. 
MKPLS  %first, it models each visual unit as a low-dimensional manifold in the feature space,. 
 describes each visual unit in manifold formate, and extract a single parameterization for each visual unit. Therefore, any further processing is done based on these parameterizations. This step isolates the inference process from the complication due to temporal variations between visual units. Yet, it uses kernel-based supervised approach for dimensionality reduction, which means that we need to investigate intensively choice of this kernel.
 %Fourth, this framework uses kernel based dimensionality reduction technique which gives the ability to investigate different manifold kernels. 
%
In principal, MKPLS pipeline has three phases: individual manifold parameterization, then latent space embedding and finally inference/classification. 

In \textbf{individual manifold parameterization}, the set of frames of the visual unit are assumed to be connected by a low-dimensional manifold in the visual feature space. Each manifold is represented by its parameterization with respect to set of basis $\{\psi_1,\psi_2,\cdots,\psi_n\}$, where $\psi_{i}(\vect{z})= exp(\vect{z},\vect{w}_i)$
%[K(\vect{z},\vect{w}_1), \cdots, K(\vect{z},\vect{w}_n)]$ . 
The parameterization is learned based on regression function $\mathcal{\gamma}(t) = \mathbf{C}^\top \Psi(t)$, and $\Psi(t)=[psi_1(t),\psi_2(t),\cdots,\psi_n(t)]$. $\mathcal{\gamma}(t) $ is chosen to minimizes a regularized loss functional in the form 
\begin{equation}
\label{eq:gamma}
    \sum_i^{n^k} \left\|\vect{x}^k_{il} - \gamma^k_l(\mathbf{z}^k_i)\right\|^2 + \lambda \; \Omega[\gamma^k_l], 
\end{equation}
where $\left\|\cdot\right\| $ is the Euclidean norm, $\Omega$ is a regularization function that enforces the smoothness in the learned function, and $\lambda$ is the regularizer that balances between fitting the training data and smoothing the learned function. When $\lambda\to 0$, the regression function over-fits the training data. The details of learning the manifold parameterization can be found in \cite{Bakry2013}. Representer theory helps to find closed form for $\mathbf{C}$ as
\begin{equation}
\label{eqn:coeff_matrix}
\mathbf{C}_k^\top  = (\mathbf{A}_k^\top\mathbf{A}_k+\lambda \mathbf{G})^{-1}\mathbf{A}_k^\top\mathbf{X}_k^\top, 
\end{equation}
where $\mathbf{A}_k$ is an $n_k \times n$ matrix with $\mathbf{A}_{(ij)}=K(\mathbf{z} _i , \mathbf{w}_j)$ %, i=1, \cdots,n_k,  j=1 \cdots n$ 
and $\mathbf{G}$ is an $ n \times n$ matrix with $\mathbf{G}_{(ij)}=K(\mathbf{w}_i , \mathbf{w}_j)$%;  i,j=1 \cdots n$
. $\mathbf{X}_k$ is the $n_k \times D$ data matrix for instance $k$. Solution for $\mathbf{C}$ is guaranteed under certain conditions on the basis functions \cite{Poggio1990:GRBF}. In this paper, we use Gaussian Radial Basis Function (Gaussian-RBF) for the kernel $K(\cdot,\cdot)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In \textbf{Latent space embedding}, kernel partial least squares (KPLS) \cite{Rosipal2002:KPLS}  is adopted for embedding the parameterizations $\{\mathbf{C}_k, k=1\cdots N\}$ into a low-dimensional latent space $\mathbb{R}^m$, as $\{\mathbf{t}_k\in \mathbb{R}^m, k=1\cdots N\}$. KPLS is supervised method, so it uses the set of labels $\{y_k, k=1\cdots N\}$ for the embedding. Supervised embedding guarantees to acheive the most concise and informative low-dimensional latent space embedding.
For any manifold $\mathcal{M}_\nu$, represented by its parameterization $\mathbf{C}_\nu$, the corresponding embedded point can be computed by
\begin{equation}
\label{eqn:embedding}
\mathbf{t_\nu = \mathbf{v}_\nu R}.
\end{equation}
Where $\mathbf{v}_\nu=K(C_\nu,.)$ (Eq~\ref{eq:cos_kernel}) is an $N$-dimensional row vector representing the similarity with all training manifold parameterizations $\{\mathbf{C}_k, k=1\cdots N\}$.
While the projection matrix $R$ is trained using KPLS algorithm presented in \cite{Rosipal2002:KPLS}.
%\begin{equation}
%\label{eqn:projection}
%\mathbf{T} = \mathbf{K}\mathbf{R}
%\end{equation} 
%Where $T$, of all embedded points, can be written as
%
%
%\subsection{Multifactor Embedding}
%As aforementioned, we have set of labeled manifold parameterizations $\{(\mathbf{C}_k,y_k);\ k=1\cdots N\}$. Consider the case where we have multiple labeling for the same manifold. Therefore, we need to deal with different classification tasks.
%% For instance, when we aim to recognize the uttered phrase, we need to label the manifolds by their phrase label. On the other hand, if we are doing speaker recognition, then manifolds have speaker labeling. In other word, manifolds have different labelings, according to different goals we need to achieve.
%In this paper, we have two simultaneous tasks: speech recognition and speaker identification.
%
%For phrase/speech recognition, the input manifolds have labeling $y^h_k, k=1\cdots N$. We can learn projection matrix $\mathbf{R}^h$ for embedded points $\mathbf{T}^h$ ({\textbf Algorithm~\ref{alg:kpls}}). 
%
%For any new manifold $\mathcal{M}_\nu$, $\mathbf{C}_\nu$ is compute (Eq~\ref{eqn:coeff_matrix}), then get the corresponding embedded point by Eq~\ref{eqn:embedding}, as $\mathbf{t}^h_\nu = \mathbf{v}_\nu \mathbf{R}^h$.
%
%For speaker identification, we have different labeling $y^p_k, k=1\cdots N$. Similarly, we learn the projection matrix $\mathbf{R}^p$ and the embedded points $\mathbf{T}^p$. For new manifold $\mathcal{M}_\nu$, we compute the parameterization $\mathbf{C}_\nu$, then get the corresponding embedded point by $\mathbf{t}^p_\nu = \mathbf{v}_\nu R^p$.
%

While in \textbf{manifold classification}, given a new manifold, parameterized by  $\mathbf{C}_\nu$, we need to classify it, i.e. to get its class label $\hat{y}_\nu$. Two classification approaches are used:
First, Regression for classification (RfC) Use regression results of KPLS
\[
%L_\nu = t_\nu T^\top\mathbf{L}
\hat{y}_\nu = \mathbf{t}_\nu \mathbf{T}^\top\mathbf{y}
\]
where $t_\nu$ is computed from Eq~\ref{eqn:embedding} (details are in \cite{Bakry2013}). 

Second choise is Support vector machines (SVM). A one-vs-all SVM classifier is learned using the set of training points $\{(\mathbf{t}_k,y_k)\in \mathbb{R}^m\times \mathbb{R};\ k=1\cdots N\}$.

%
%\section{Single frame classification}
%\section{Toward continuous speech recognition}
%In the section \ref{sec:classify}, we assumed that we have all frames of the new sequence $\mathcal{S}^\nu$ are avaialble. Toward continuous speech recognition, we have to consider the case of classifying the phrase/speaker from solely single or couple of frames. 
%
%For doing that, we need to have generative model. Recipe of generative model is 1) descriptor for single frame 2) some measurement for how sure we are that the image in hand belong to certain sequence 3) classifier for he choosen sequence to know the word and the speaker of this speech video.
%We can do that using sampling method. So we sample from both the 
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

